ORCa: Glossy Objects as Radiance Field Cameras

Reflections on glossy objects contain valuable and hidden information about the surrounding environment. By converting these objects into cameras, we can unlock exciting applications, including imaging beyond the camera's field-of-view and from seemingly impossible vantage points, e.g. from reflections on the human eye. However, this task is challenging because reflections depend jointly on object geometry, material properties, the 3D environment, and the observer viewing direction. Our approach converts glossy objects with unknown geometry into radiance-field cameras to image the world from the object's perspective. Our key insight is to convert the object surface into a virtual sensor that captures cast reflections as a 2D projection of the 5D environment radiance field visible to the object. We show that recovering the environment radiance fields enables depth and radiance estimation from the object to its surroundings in addition to beyond field-of-view novel-view synthesis, i.e. rendering of novel views that are only directly-visible to the glossy object present in the scene, but not the observer. Moreover, using the radiance field we can image around occluders caused by close-by objects in the scene. Our method is trained end-to-end on multi-view images of the object and jointly estimates object geometry, diffuse radiance, and the 5D environment radiance field.

==> tables/comparison_table.tex <==
\begin{table*}
\centering
\footnotesize
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  width = 0.9\linewidth,
  colspec = {Q[160]Q[231]Q[202]Q[175]Q[167]},
  hline{1,8} = {-}{0.08em},
  hline{2} = {-}{0.05em},
}
Approach             & Input               & {Scene \\Geometry~} & {Algorithm\\Type} & {Environment\\Dimensions} \\
Neural Illum. \cite{song2019neural}       & Single RGB          & Normals             & Supervised        & 2D                           \\
Lighthouse \cite{srinivasan2020lighthouse}          & Stereo RGB pair     & Multi-plane Image   & Supervised        & 5D                            \\
NeRFactor \cite{zhang2021nerfactor}             & Multi-view RGB      & Volumetric Albedo   & Semi-supervised   & 2D                           \\
RefNeRF \cite{verbin2022refnerf}             & Multi-view RGB      & Volumetric Albedo   & Self-supervised   & 2D                           \\
PANDORA \cite{dave2022pandora}             & Multi-view RGB+Pol. & Neural SDF          & Self-supervised   & 2D                            \\
\textbf{ORCA (Ours)} & Multi-view RGB      & Neural SDF          & Self-supervised   & 5D                          
\end{tblr}
}
\caption{\textbf{Comparison of environment estimation approaches}. Neural Illum \cite{song2019neural}, Lighthouse \cite{srinivasan2020lighthouse}, NeRFFactor \cite{zhang2021nerfactor} train on datasets of natural illumination maps to regularize ill-posedness of environment estimation. PANDORA \cite{dave2022pandora} and RefNeRF\cite{verbin2022refnerf} exploit multi-view reflections on object but approximate surrounding environment is infinitely far away and model it with a flat 2D map. From multi-view reflections, ORCa converts the object surface into virtual sensor and extracts 5D radiance field of the environment. }
\end{table*}
